Alternating Mahalanobis Distance Minimization for Stable and Accurate CP Decomposition

CP decomposition (CPD) is prevalent in chemometrics, signal processing, data mining and many more fields. While many algorithms have been proposed to compute the CPD, alternating least squares (ALS) remains one of the most widely used algorithm for computing the decomposition. Recent works have introduced the notion of eigenvalues and singular values of a tensor and explored applications of eigenvectors and singular vectors in areas like signal processing, data analytics and in various other fields. We introduce a new formulation for deriving singular values and vectors of a tensor by considering the critical points of a function different from what is used in the previous work. Computing these critical points in an alternating manner motivates an alternating optimization algorithm which corresponds to alternating least squares algorithm in the matrix case. However, for tensors with order greater than equal to $3$, it minimizes an objective function which is different from the commonly used least squares loss. Alternating optimization of this new objective leads to simple updates to the factor matrices with the same asymptotic computational cost as ALS. We show that a subsweep of this algorithm can achieve a superlinear convergence rate for exact CPD with known rank and verify it experimentally. We then view the algorithm as optimizing a Mahalanobis distance with respect to each factor with ground metric dependent on the other factors. This perspective allows us to generalize our approach to interpolate between updates corresponding to the ALS and the new algorithm to manage the tradeoff between stability and fitness of the decomposition. Our experimental results show that for approximating synthetic and real-world tensors, this algorithm and its variants converge to a better conditioned decomposition with comparable and sometimes better fitness as compared to the ALS algorithm.

==> cond.tex <==
 \begin{lemma}
 \label{lem:kh_norm}
 Norm of a Khatri-Rao product of two matrices $\mat A$ and $\mat B$ is at most the product of their respective norms, i.e.,
 \[ \|\mat A \odot \mat B\| \leq \|\mat A\| \|\mat B\|. 
 \]
 \end{lemma}
 \begin{proof}
 Let $\mat U_A \mat S_A \mat V^T_A$ and $\mat U_B \mat S_B \mat V^T_B$ be the full singular value decomposition of $\mat A$ and $\mat B$ respectively. Then,
 \[ \mat A \odot \mat B = (\mat U_A \otimes \mat U_B)(\mat S_A \otimes \mat S_B)(\mat V^T_A \odot \mat V^T_B).
 \]
 Since $\mat U_A,\mat U_B,\mat V_A,$ and $ \mat V_B$ are orthogonal matrices, and Khatri-Rao product of two orthogonal matrices is orthonormal. Therefore,
 \[\|\mat A \odot \mat B\| \leq \|\mat S_A \otimes \mat S_B\| \leq \|\mat S_A\|\|\mat S_B\|,
 \]
 \[
 \|\mat A \odot \mat B\| \leq \|\mat A\|\|\mat B\|.
 \]
 \end{proof}

 \begin{lemma}
 \label{lem:kh_norm_low}
 Frobenius Norm of a Khatri-Rao product of two matrices $\mat A$ and $\mat B$ is at least a constant times the norm of one of the matrix divided by the norm of the Moore-Penrose inverse of the other, i.e.,
 \[ \|\mat A \odot \mat B\|_2 \geq c\frac{\|\mat A\|_2}{ \|\mat B^\dagger\|_2}. 
 \]
 \end{lemma}
 \begin{proof}
 Let $\mat U_A \mat S_A \mat V^T_A$ and $\mat U_B \mat S_B \mat V^T_B$ be the full singular value decomposition of $\mat A$ and $\mat B$ respectively. Then,
 \[\|\mat A \odot \mat B\|_2  = \max_{\|\vcr x\| = 1}\|\vcr x^T(\mat A \odot \mat B) \|= \max_{\|\vcr x\| = 1}\| \vcr x^T (\mat U_A \otimes \mat U_B) (\mat S_A \otimes \mat S_B)(\mat V^T_A \odot \mat V^T_B)  \|.
 \]
 Now, let $\vcr u^B_{k}$ and $\sigma^B_{k}$ be the $kth$ singular value of $\mat B$ and the corresponding left singular vector respectively. Similarly let $\vcr u^A_{\text{max}}$ and $\sigma^A_{\text{max}}$ be the maximum singular value of $\mat A$ and the corresponding left singular vector. 

 \begin{align*}
     \max_{\|\vcr x\| = 1}\|\vcr x^T(\mat A \odot \mat B) \| &\geq\max_k\| (\vcr u^A_{\text{max}} \otimes  \vcr u^B_{k})^T(\mat U_A \otimes \mat U_B) (\mat S_A \otimes \mat S_B)(\mat V^T_A \odot \mat V^T_B)\| \\
     &=\max_k\|   \sigma^A_{\text{max}}\sigma^B_{k}(\vcr v_1 \ast \vcr v_k) \|
 \end{align*}

 \end{proof}

 \begin{lemma}
 \label{lem:cond_pinv}
 The relative conditioning of computing the Moore-Penrose inverse of a matrix $\mat A \in \mathbb{C}^{m \times n}$ with a perturbation $\mat \Delta$ such that rank($\mat A + \mat \Delta)= \min(m,n)$ is at most~\cite{stewart1977perturbation}
 \[2\|\mat A\|\|(\mat A + \mat \Delta)^\dagger\|_2\]
 i.e.,
 \[\frac{\|(\mat A + \mat{\Delta})^{\dagger} - \mat A^{\dagger}\|}{\|\mat A^{\dagger}\|}\leq 2\|\mat A\|\|(\mat A + \mat \Delta)^\dagger\|_2\frac{\|\mat \Delta\|}{\|\mat A\|}.\]
 \end{lemma}
 \begin{proof}
 Theorem 3.8 of~\cite{stewart1977perturbation}. \end{proof}

 \begin{theorem}
 \label{thm:ALS_cond}
 The relative conditioning of computing the Moore-Penrose inverse of the Khatri-Rao product of two full rank matrices $\mat A$ and $\mat B$ with a perturbation $\mat \Delta$ which does not alter the rank of either of the matrices  is 
 \[
 \frac{\|\big((\mat A + \mat{\Delta}) \odot (\mat B + \mat{\Delta})\big)^\dagger- (\mat{A}\odot \mat{B})^\dagger\|}{\|\mat (\mat A \odot \mat B)^\dagger\|} = O\Big(\|\mat A\| \|\mat B\| \|(\mat A +\mat \Delta)^\dagger \|_2  \|(\mat B +\mat \Delta)^\dagger \|_2\Big) \epsilon,
 \]
 where $\epsilon = \max (\frac{\|\mat \Delta\|}{\|\mat A\|},\frac{\|\mat \Delta\|}{\|\mat B\|})$.
 \end{theorem}
 \begin{proof}
 We can use Lemma~\ref{lem:cond_pinv}, by using $\mat \Delta' = (\mat \Delta \odot \mat B) + (\mat A \odot \mat \Delta) + (\mat \Delta \odot \mat \Delta)$ and $\mat Z = \mat A \odot \mat B$,
 \[ \frac{\|(\mat Z + \mat \Delta')^\dagger - \mat Z^\dagger\|}{\|\mat Z^\dagger\|} \leq 2 \|\mat Z\|\|(\mat Z + \mat \Delta ')^\dagger\|_2 \frac{\|\mat \Delta '\|}{\|\mat Z \|},
 \]
 which  implies that
 \[\frac{\|\big((\mat A + \mat{\Delta}) \odot (\mat B + \mat{\Delta})\big)^\dagger- (\mat{A}\odot \mat{B})^\dagger\|}{\|\mat (\mat A \odot \mat B)^\dagger\|} \leq 2\|\mat A \odot \mat B\| \|((\mat A + \mat \Delta) \odot (\mat B + \mat \Delta))^\dagger\|_2\frac{\|\mat \Delta' \|}{\|\mat A \odot \mat B\|}. \]
 Using triangular inequality and Lemma~\ref{lem:kh_norm},
 \begin{align*}
     \|\mat \Delta'\| &= \|(\mat \Delta \odot \mat B) + (\mat A \odot \mat \Delta) + (\mat \Delta \odot \mat \Delta) \| \\
     &\leq \|\mat \Delta \odot \mat B \| + \|\mat A \odot \mat \Delta \| + \|\mat \Delta \odot \mat \Delta \| \\
     &\leq \|\mat A\| \|\mat B\| \big( \frac{\|\mat \Delta \|}{\|\mat A\|}+\frac{\|\mat \Delta \|}{\|\mat B\|} + \frac{\|\mat \Delta\|^2}{
    \|\mat A\|\| \mat B\|} \big).
 \end{align*}
 
Ignoring the quadratic term in $\|\mat \Delta\|$ and using the above result, we get
 \[
 \frac{\|((\mat A + \mat{\Delta}) \odot(\mat B + \mat{\Delta}))^\dagger - (\mat{A}\odot \mat B)^{\dagger}\|}{\|(\mat A \odot \mat B)^\dagger\|} = O\Big(\|\mat A\| \|\mat B\| \|(\mat A +\mat \Delta)^\dagger \|_2  \|(\mat B +\mat \Delta)^\dagger \|_2\Big)\epsilon.\]
 \end{proof}


 \begin{theorem}
 \label{thm:M_cond}
 The relative conditioning of computing the Khatri-Rao product of Moore-Penrose inverse transpose of two matrices $\mat A$ and $\mat B$ with a perturbation $\mat \Delta$ that does not alter the rank of either of the matrices is
 \[
 \frac{\|(\mat A + \mat{\Delta})^{\dagger T} \odot (\mat B + \mat{\Delta})^{\dagger T}- (\mat{A}^{\dagger T}\odot \mat{B}^{\dagger T})\|}{\|\mat A^{\dagger T} \odot \mat B^{\dagger T}\|} = O\Big(\frac{\|\mat A^\dagger\|\|\mat B^\dagger\|}{\|\mat A^{\dagger T}\odot \mat B^{\dagger T}\|}\big( \|\mat A\|\|(\mat A + \mat \Delta)^\dagger\|_2 + \|\mat B\|\|(\mat B + \mat \Delta)^\dagger\|_2\big) \Big) \epsilon,
 \]
 where $\epsilon = \max (\frac{\|\mat \Delta\|}{\|\mat A\|},\frac{\|\mat \Delta\|}{\|\mat B\|})$.
 \end{theorem}
 \begin{proof}
 From Lemma~\ref{lem:cond_pinv} we know that 
 \[ \|(\mat A + \mat{\Delta})^{\dagger T} \odot (\mat B + \mat{\Delta})^{\dagger T}\| = \| (\mat A^{\dagger T} + \mat \Delta_A) \odot (\mat B^{\dagger T} + \mat \Delta_B)\|.
 \]
 We can use triangular inequality and Lemma~\ref{lem:kh_norm} to show that
 \[\| (\mat A^{\dagger T} + \mat \Delta_A) \odot (\mat B^{\dagger T} + \mat \Delta_B)- (\mat{A}^{\dagger T}\odot \mat{B}^{\dagger T})\| = O \Big(\|\mat A^\dagger \| \|\mat B^\dagger\|\big(\frac{\|\mat \Delta_A \|}{\|\mat A^\dagger \|} +\frac{\|\mat \Delta_B \|}{\|\mat B^\dagger \|} \big)\Big).
 \]
 Now, using the bounds from Lemma~\ref{lem:cond_pinv},
 \[\frac{\|\mat \Delta_A \|}{\|\mat A^\dagger \|} +\frac{\|\mat \Delta_B \|}{\|\mat B^\dagger \|}  \leq  \|\mat A\|\|(\mat A + \mat \Delta)^\dagger\|_2 \frac{\|\mat \Delta \|}{\|\mat A\|} + \|\mat B\|\|(\mat B + \mat \Delta)^\dagger\|_2\frac{\|\mat \Delta \|}{\|\mat B\|}
 \]
 Hence, we get
 \[
 \frac{\|(\mat A + \mat{\Delta})^{\dagger T} \odot (\mat B + \mat{\Delta})^{\dagger T}- (\mat{A}^{\dagger T}\odot \mat{B}^{\dagger T})\|}{\|\mat A^{\dagger T} \odot \mat B^{\dagger T}\|} = O\Big(\frac{\|\mat A^\dagger\|\|\mat B^\dagger\|}{\|\mat A^{\dagger T}\odot \mat B^{\dagger T}\|}\big( \|\mat A\|\|(\mat A + \mat \Delta)^\dagger\|_2 + \|\mat B\|\|(\mat B + \mat \Delta)^\dagger\|_2\big) \Big) \epsilon.
 \]
 \end{proof}

The objective~\ref{eq:obj_mnorm} can be rewritten as \begin{align}
    \frac{1}{2}\|\tsr{X}\times_1\mat A^{(1)\dagger} \times_2 \ldots \times_N \mat A^{(N)\dagger} - \tsr{I} \|_F^2,
\end{align}
where $\tsr{I}$ is an $N$ order binary tensor with each mode length as $R$ and ones on the diagonal of the tensor.

==> motiv.tex <==
To introduce our alternating optimization scheme, we first consider the case of finding an exact CP decomposition of a low rank tensor. Let  $\tsr{X} \in \mathbb{R}^{I_1 \times I_2 \times I_3}$ be the input tensor with 
CP rank $R$ with $R< I_n, \forall n \in \{1,2,3\}$. Let $\mat{A}^{(1)}$, $\mat{A}^{(2)}$, and $\mat{A}^{(3)}$ be  the factor matrices initialized with random numbers. Also, assume that all the factors are full matrix rank. 
Consider the linear least squares subproblem for each factor matrix,
\begin{equation}
    \mat{A}^{(1)}_{\text{new}}(\mat{A}^{(3)}\odot \mat{A}^{(2)})^T \cong \mat{X}_{(1)}.
    \label{eq:llsq}
\end{equation}
Instead of solving this linear least squares problem exactly by projecting with the pseudoinverse of \(\mat{A}^{(3)}\odot \mat{A}^{(2)}\), as in standard ALS, we instead project onto the (generally different) left inverse $\Big(\mat{A}^{(3)\dagger T}\odot\mat{A}^{(2)\dagger T}\Big)^T$,
\[\mat{A}^{(1)}_{\text{new}}\underbrace{\Big(\mat{A}^{(3)}\odot \mat{A}^{(2)}\Big)^T\Big(\mat{A}^{(3)\dagger T}\odot\mat{A}^{(2)\dagger T}\Big)}_{\mat I} = \mat{X}_{(1)}\Big(\mat{A}^{(3)\dagger T}\odot\mat{A}^{(2)\dagger T}\Big).\] 
We obtain an algorithm with an update rule that is straight forward to compute,
\begin{align}
\label{eq:Mnorm_update}
    \mat{A}^{(1)}_{\text{new}} = \mat{X}_{(1)} \Big(\mat{A}^{(3)\dagger T}\odot\mat{A}^{(2)\dagger T}\Big).
\end{align}
An advantage of this update rule over standard ALS, is its capability to achieve high-order convergence.
Assuming the factor matrices are some perturbation $\mat{\Delta}$ away from a true CP decomposition $\mat{A}^{(1)}$, $\mat{A}^{(2)}$, $\mat{A}^{(3)}$, we show in Section~\ref{subsec:mnorm_conv} that
\[\mat{A}^{(1)}_{\text{new}} = \mat{X}_{(1)} \Big(\big(\mat{A}^{(3)} + \mat{\Delta}\big)^{\dagger T}\odot\big(\mat{A}^{(2)} + \mat{\Delta}\big)^{\dagger T}\Big) = \mat{A}^{(1)} \mat{D} + O(\|\mat{\Delta}\|^2),\]
for some diagonal matrix $\mat{D}$.
Since, the column scaling of factor matrix is indetermiante, our analysis implies that the new update rule can achieve a convergence rate of $(1+\sqrt{5})/2$ per subsweep (and yet higher order if the tensor is higher order).

When considering the more general setting of approximating the tensor by a low rank CP decomposition,
the above update may be viewed as a method for
minimization of the error in a different norm,
\begin{equation}
    \min_{\mat{A}^{(1)}_{\text{new}}}\|\mat{X}_{(1)} - \mat{A}^{(1)}_{\text{new}}(\mat{A}^{(3)}\odot \mat{A}^{(2)})^T\|_{\mat{M}},
    \label{eq:Mnorm_min}
\end{equation}
where  $\mat{M} = \big(\mat{A}^{(3)}\mat{A}^{(3)T} \otimes \mat{A}^{(2)}\mat{A}^{(2)T} \otimes \mat{A}^{(1)}\mat{A}^{(1)T}  \big)^\dagger $.
Specifically, in Section~\ref{sec:mnorm}, we show that \eqref{eq:Mnorm_update} corresponds to finding the minimizer $\mat{A}^{(1)}$ to \eqref{eq:Mnorm_min} with $\mat{A}^{(2)}$ and $\mat{A}^{(3)}$ fixed.

Minimization under this new metric tends to result in well-conditioned factors.
%The main reason for this is that 
The minimized function involves products with the pseudoinverses of the factors, which will generally be large if they have large norm.
Consequently, the factors are unlikely to have small singular values.
We provide intuition for this property in the case of matrix decomposition case, which generalizes naturally to higher-order tensors.
For approximate factorization of a matrix $\mat X$ with factors $\mat A$ and $\mat B$, our method minimizes the objective function,
\[f(\mat A, \mat B) = \|\mat A^\dagger \mat X \mat B^\dagger{}^T - \mat I\|_F.\]
We can rewrite this objective function in terms of the residual error of the decomposition, $\mat R = \mat X - \mat A \mat B^T$, as
\[f(\mat A, \mat B)=\|\mat A^{\dagger}\mat R \mat{B}^{\dagger}{}^T \|_F = \|(\mat A^\dagger \otimes \mat B^\dagger) \text{vec}(\mat R)\|_2.\]
Hence, during optimization, when the residual $\mat R$ is large and possibly full-rank, the objective function will generally be correlated with $\|\mat A^\dagger \otimes \mat B^\dagger\|_2=\|\mat A^\dagger\|_2\cdot \| \mat B^\dagger\|_2$.
Consequently, as the objective value decreases during optimization, the minimum singular values of the computed factors $\mat A$ and $\mat B$ tend to be relatively large, yielding good conditioning.
In Section~\ref{sec:exp}, we provide numerical evidence showing that the new method yields much better conditioned factors and iterates than standard ALS.


%be more well-conditioned.
%Compared to the pseudoinverse in standard ALS, the left inverse projection may not change as rapidly when $\mat A^{(2)}$ and $\mat A^{(3)}$ are peturbed, since
%{\small
%\begin{align*}
%\frac{\|((\mat A^{(3)} + \mat{\Delta}) \odot(\mat A^{(2)} + \mat{\Delta}))^\dagger - (\mat{A}^{(3)}\odot \mat{A}^{(2)})^{\dagger}\|}{\|(\mat{A}^{(3)}\odot \mat{A}^{(2)})^{\dagger}\|} &= O\Big(\kappa^2(\mat A^{(3)}) \kappa^2(\mat A^{(2)}) \Big)\epsilon,
%\end{align*}}
%\noindent while
%{\small
%\begin{align*}
%\frac{\|(\mat A^{(3)} + \mat{\Delta})^{\dagger T} \odot(\mat A^{(2)} + \mat{\Delta})^{\dagger T} - (\mat{A}^{(3)\dagger T}\odot \mat{A}^{(2)\dagger T})\|}{\|\mat{A}^{(3)\dagger T}\odot \mat{A}^{(2)\dagger T} \|} &= O\Big(\kappa(\mat A^{(3)}) \kappa(\mat A^{(2)}) (\kappa (\mat A^{(3)})+\kappa(\mat A^{(2)}))  \Big) \epsilon,
%\end{align*}
%}
%where $\epsilon =\min (\|\mat \Delta\|/\|\mat A^{(3)}\|, \|\mat \Delta\|/\|\mat A^{(2)}\|)$. Consequently, the distance among points (values of $\mat{A}^{(1)}$, $\mat{A}^{(2)}$, and $\mat{A}^{(3)}$) is less variable to perturbations.
%Experimentally, in approximate CP, we observe that the condition numbers of the factor matrices often grow in ALS (the ill-conditioning of the update rules compounds ill-conditioning of the factor matrices) leading to an increase in CPD condition number (cite), while minimizing the new distance metric typically leads to well-conditioned factor matrices resulting in a smaller CPD condition number.



==> sing.tex <==
\textcolor{red}{navjot: Change this} As we have shown in Section~\ref{sec:conv}, Algorithm~\ref{alg:mnorm_basic} achieves local convergence to an exact CP tensor decomposition.
However, when the true rank of the tensor is greater than the number of columns in sought-after factors, the algorithm generally does not converge to local minima of the decomposition residual error.
In our experiments, we observe that the method converges to a fixed point irrespective of the rank of the underlying tensor.
We characterize these fixed points in terms of the pseudoinverses of the factors, observing that these satisfy a certain orthonormality condition with respect to the tensor.

\subsection{Singular values and vectors of a tensor}
We introduce a formulation to compute the singular values and singular vectors of a tensor $\tsr{X}$. Let $f_{\tsr{X}} : \mathbb{R}^{I_1} \times \ldots \times \mathbb{R}^{I_N} \to \mathbb{R}$ denote the multilinear functional associated with the tensor given as
\[f_{\tsr{X}}(\vcr v^{(1)},\ldots, \vcr{v}^{(N)}) = \sum_{i_1\ldots i_N}x_{i_1\ldots i_N}\prod_{j=1}^N v^{(j)}_{i_j}.\]
We define the singular vectors of a tensor using the critical points of the functional $L: \mathbb{R}^{I_1} \times \ldots \times \mathbb{R}^{I_N} \to \mathbb{R}$,
\[L(\vcr v^{(1)},\ldots, \vcr{v}^{(N)}) = f_{\tsr{X}}(\vcr v^{(1)},\ldots, \vcr{v}^{(N)}) - \frac{1}{2}\sum_{i=1}^N\log\|\vcr{v}^{(i)}\|^2_2.
\]
The functional $L$ is continuously differentiable for nonzero $\vcr{v}^{(i)}$ for all $i$, and at the critical points of $L$, we have
\[
f_{\tsr{X}}(\vcr v_i^{(1)},\ldots, \vcr v_i^{(n-1)}, \mat I_{I_n}, \vcr v_i^{(n+1)},\ldots, \vcr v_i^{(N)}) = \frac{\vcr{v}^{(n)}}{\|\vcr{v}^{(n)}\|_2^2}, \quad \forall i \in \{1,\dots,N\}.
\]
We now define $\vcr{\varphi}^{(i)} = \frac{\vcr v^{(i)}}{\|\vcr v^{(i)} \|_2}$ as the mode $i$ singular vector and $\prod_{i=1}^N \|\vcr{v}^{(i)}\|_2 = \frac{1}{\sigma}$ as the singular value of the tensor $\tsr{X}$. \textcolor{red}{TODO: Add matrix things, Do we want general norm? }

\textcolor{red}{TODO: New section for inverse operation of matricization of T}

\subsection{Fixed Point Orthogonality Conditions}

When Algorithm~\ref{alg:mnorm_basic} converges to a fixed point,
the factors and pseudoinverses of the factors $\mat{U}^{(n)} = \mat{A}^{(n)}{}^\dagger$ satisfy
\[\mat{A}^{(n)} = \mat{X}^{(N)}_{(n)}\bigg(\bigodot_{m=1,m\neq n}^N \mat{U}^{(m)}{}^T\bigg)\]
for all $n\in\{1,\ldots N\}$.
Premultiplying by $\mat{U}^{(n)}$, the above conditions imply
\[\mat{I} = \mat{U}^{(n)}\mat{X}^{(N)}_{(n)}\bigg(\bigodot_{m=1,m\neq n}^N \mat{U}^{(m)}{}^T\bigg).\]
We may rewrite these in terms of the multilinear function associated with the tensor
as a set of orthonormality conditions on the rows of each $\mat{U}^{(n)}$,
\[f_{\tsr{X}}(\vcr u_i^{(1)},\ldots, \vcr u_i^{(n-1)}, \vcr u_j^{(n)}, \vcr u_i^{(n+1)},\ldots, \vcr u_i^{(N)}) = \delta_{ij},\]
where $\delta_{ij}$ is the Kronecker delta.
These conditions imply that each pair of columns of $\mat{U}^{(n)}$ should be nearly orthogonal, and hence the factor matrix $\mat{A}^{(n)}$ should be well-conditioned.

For a tensor with exact rank $R'\leq s =\min_{n} I_n$, any matching choice of $R\leq R'$ rows of the pseudoinverse of each of the exact factor matrices satisfies the above orthonormality conditions.
In particular, if $\tsr{X} = [\![ \mat{\hat{A}}^{(1)}, \cdots , \mat{\hat{A}}^{(N)} ]\!]$ and the pseudoinverses of the exact factors are $\mat{\hat{U}}^{(n)} = \mat{\hat{A}}^{(n)}{}^\dagger$,
\[f_{\tsr{X}}(\hat{\vcr u}_i^{(1)},\ldots, \hat{\vcr u}_i^{(n-1)}, \hat{\vcr u}_j^{(n)}, \hat{\vcr u}_i^{(n+1)},\ldots, \hat{\vcr u}_i^{(N)}) = \langle \underbrace{\mat{\hat{A}}^{(n)}{}^T\hat{\vcr u}_j^{(n)}}_{\vcr{e}_j}, \ast_{m=1,m\neq n}^N\underbrace{\mat{\hat{A}}^{(n)}{}^T\hat{\vcr u}_i^{(n)}}_{\vcr e_i}\rangle.\]
However, such a collection of pseudoinverse rows is generally not a fixed point of the iterative scheme in Algorithm~\ref{alg:mnorm_basic}, as the projected conditions are necessary but not sufficient for this.
For a tensor with rank $R'<R$, a set of $R$ vectors that satisfy orthonormality do not exist, since $\mat{X}^{(N)}_{(n)}\Big(\bigodot_{m=1,m\neq n}^N \mat{U}^{(1)}{}^T\Big)$ cannot be full rank.
Our numerical results suggest that fixed points of the method exist also when the true rank exceeds the dimension ($R>s$).
%, it is not clear if such a fixed point always exists, but numerical experiments suggest the method can find a fixed point for such tensors as well.
